Periodicity in tilings

Tilings and tiling systems are an abstract concept that arise both as a computational model and as a dynamical system. In this paper, we characterize the sets of periods that a tiling system can produce. We prove that up to a slight recoding, they correspond exactly to languages in the complexity classes $\nspace{n}$ and $\cne$.

==> figures/exemple_interdits.tex <==
\begin{tikzpicture}[scale=0.5]
 \filldraw[color=red] (0,0) rectangle (1,1);
 \filldraw[color=blue!20] (1,0) rectangle (2,1);

 \filldraw[color=red] (3,0) rectangle (4,1);
 \filldraw[color=blue!20] (4,0) rectangle (5,1);
 
 \filldraw[color=red] (6,0) rectangle (7,1);
 \filldraw[color=blue!20] (6,1) rectangle (7,2);
\end{tikzpicture}


